Modeling Reusable, Platform-Independent Robot Assembly Processes

Smart factories that allow flexible production of highly individualized goods require flexible robots, usable in efficient assembly lines. Compliant robots can work safely in shared environments with domain experts, who have to program such robots easily for arbitrary tasks. We propose a new domain-specific language and toolchain for robot assembly tasks for compliant manipulators. With the LightRocks toolchain, assembly tasks are modeled on different levels of abstraction, allowing a separation of concerns between domain experts and robotics experts: externally provided, platform-independent assembly plans are instantiated by the domain experts using models of processes and tasks. Tasks are comprised of skills, which combine platform-specific action models provided by robotics experts. Thereby it supports a flexible production and re-use of modeling artifacts for various assembly processes.

==> commands/biblatex <==
#!/bin/bash
# biblatex runs latex and bibtex as often as necessary,
# It detects citation problems and in this case reruns bibtex.
# It detects label-changes and reruns latex (up to 3 times),
# However, if labels are defined twice, it always runs latex three times.
#
# REMARK: a slightly changed bibliography does not cause a bibtex call
# because this is not detected.
#
# BUG: (from latex:) A changed (sub..) section name is not recognised and
# therefore the last run incorporating the changed table of contents (toc)
# not executed.
#

if [ $# -eq 1 ]
then
    datei=`dirname $1`/`basename $1 .tex`
    latex=latex
elif [ $# -eq 2 ]
then
    datei=`dirname $2`/`basename $2 .tex`
    latex=$1
else
    echo 'usage: $0 [latex-command] latex-file[.tex]'
    exit 1
fi

temp=$datei.blx

echo $0: $latex $datei  \(pass 1 is always performed\)
$latex $datei
error=$?
if [ $error -ne 0 ]
then exit $error
fi

  # part 1: expand of all .aux files in $temp
  grep '\\@input{' $datei.aux \
    | sed -e 's/\\@input{//g' -e 's/}//g' > $temp.2
  echo $0: Expanding .aux-files: $datei.aux `cat $temp.2`
  cat $datei.aux `cat $temp.2` > $temp
  rm $temp.2
  
# is there a bibliography entry? (else skip 2-5)
grep '\\bibdata{' $temp >/dev/null
if [ $? -eq 0 ]
then

  # part 2: actual and desired citations in $temp.4 and $temp.5
  grep '\\citation{' $temp \
    | sed -e 's/\\citation{//g' -e 's/}//g' \
    | sort -u > $temp.4
  grep '\\bibcite{' $temp \
    | sed -e 's/\\bibcite{//g' -e 's/}.*$//g' \
    | sort -u > $temp.5

  echo $0: Required citations: `cat $temp.4 | wc -l`
  echo $0: Given citations: `cat $temp.5 | wc -l`
  diff $temp.4 $temp.5 >/dev/null
  diffs=$?
  rm $temp.4 $temp.5

  # part 3: check are there citation problems?
  grep 'Citation .* undefined' $datei.log >/dev/null
  citations=$?

  # part 4: is a bib-file newer than the bbl-file?
  grep '\\bibdata{' $temp \
    | sed -e 's/\\bibdata{//g' -e 's/}/.bib/g' -e 's/,/.bib\
/g' > $temp.2
  bibfilenew=0
  for i in `cat $temp.2`
  do
     if [ $i -nt $datei.bbl ]
     then 
        bibfilenew=1
     fi
  done
  rm $temp.2

  # part 5: execute bibtex
  if [ $citations -eq 0 -o $diffs -ne 0 -o $bibfilenew -ne 0 ]
  then
    echo $0: bibtex $datei \(citation problems and bibliography entries\)
    bibtex $datei
    error=$?
    if [ $error -ne 0 ]
    then exit $error
    fi

    echo $0: $latex $datei \(because of citation problems\)
    $latex $datei
    error=$?
    if [ $error -ne 0 ]
    then exit $error
    fi
  fi

fi

# part 6: three times repeat, to get cross-references right
for i in 1 2 3
do
    grep 'Rerun to get cross-references right' $datei.log >/dev/null
    if [ $? -eq 0 ]
    then
        echo $0: $latex $datei \(to get cross-references right, pass $i\)
        $latex $datei
        error=$?
        if [ $error -ne 0 ]
        then exit $error
        fi
    fi
done



==> makefile <==
######################################################################
# 
# makefile 	V3.1
#  fuer normale Latex-Projekte mit ppt-Bildern
#
# Anzupassen sind: TARGET, SOURCES, PICS, LISTINGS
#   (und sonst normalerweise nichts, also nur die
#   folgenden vier Zeilen)

# Ziel:
TARGET=paper.pdf

SOURCES=paper.tex tex/*.tex

PICS=

BIB=paper.bib

LISTINGS=

######################################################################
# alles zusammen (und am Ende einige Hilfsinfos ausgeben)
all: at-start check-commands $(TARGET) warnings
	@echo --------------------------
	@echo ghostview $(TARGET) \&
	@echo gmake clean 

# Zu Beginn einige Hilfsinfos ausgeben
at-start:
	@echo target: $(TARGET)
	@echo tex-files: $(SOURCES)
	@echo pics: $(PICS)
	@echo listings: $(LISTINGS)

.SUFFIXES: $(SUFFIXES) .pptx .gflag .tex .eps .ps .pdf

.PHONY : all at-start clean warnings check-commands biblatex

# %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
# generate pics from ppt:
.pptx.gflag:
	mkdir -p gen
	@echo do ppt2eps $< -o gen
	@java -jar commands/ostp-client-ppt2eps-2.3.4.jar $< -o gen
	# ppt2eps $< -o gen
	touch $@

# %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
# make only the pics
pics: $(PICS:.pptx=.gflag)

# %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
$(TARGET): $(SOURCES) $(BIB) $(PICS:.pptx=.gflag) $(LISTINGS)
	./commands/biblatex "pdflatex -synctex=-1" $(TARGET:.pdf=)

# %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
# ueberfluessigen Schrott loeschen
clean:
	@rm -f $(TARGET:.pdf=.aux) $(TARGET:.pdf=.blx) $(TARGET:.pdf=.dvi)
	@rm -f $(TARGET:.pdf=.idx) $(TARGET:.pdf=.log) $(TARGET:.pdf=.pdf)
	@rm -f $(TARGET:.pdf=.toc) $(TARGET:.pdf=.pdf) $(TARGET:.pdf=.blg)
	@rm -f $(TARGET:.pdf=.synctex)
	@rm -f $(TARGET:.pdf=.out)
	@rm -f $(SOURCES:.tex=.aux)
	@rm -f $(PICS:.pptx=.gflag)
	@rm -f *.bak *~
    
clean-pdf:
	@rm -f $(TARGET:.pdf=.aux) 
  
cleanall: clean clean-pdf
	@rm -f $(TARGET:.pdf=.bbl)


# %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
# latex-Warnings nochmal kompakt ausgeben:
warnings:
	@-echo -------------------------- Warnings from bib
	@-grep arning- $(TARGET:.pdf=.blg)
	@-echo -------------------------- Warnings from latex
	@-grep arning: $(TARGET:.pdf=.log)

open:
	pdfopen --file=$(TARGET)

text: clean-pdf $(SOURCES) $(BIB) $(PICS:.pptx=.gflag) $(LISTINGS)
	./commands/biblatex pdflatex $(TARGET:.pdf=)
   
# %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
# check, ob Kommandos existieren 
COMMANDS=latex bibtex grep rm # biblatex
check-commands: 
	@for i in $(COMMANDS); do\
	   which $$i > /dev/null || \
	     (echo "ERROR: command $$i not available!"; \
	      echo "   please install this command first, e.g. from"; \
	      echo "   http://www.sselab.de/?"; \
	      exit -1); \
	   done


